In-N-Out: Towards Good Initialization for Inpainting and Outpainting

In computer vision, recovering spatial information by filling in masked regions, e.g., inpainting, has been widely investigated for its usability and wide applicability to other various applications: image inpainting, image extrapolation, and environment map estimation. Most of them are studied separately depending on the applications. Our focus, however, is on accommodating the opposite task, e.g., image outpainting, which would benefit the target applications, e.g., image inpainting. Our self-supervision method, In-N-Out, is summarized as a training approach that leverages the knowledge of the opposite task into the target model. We empirically show that In-N-Out -- which explores the complementary information -- effectively takes advantage over the traditional pipelines where only task-specific learning takes place in training. In experiments, we compare our method to the traditional procedure and analyze the effectiveness of our method on different applications: image inpainting, image extrapolation, and environment map estimation. For these tasks, we demonstrate that In-N-Out consistently improves the performance of the recent works with In-N-Out self-supervision to their training procedure. Also, we show that our approach achieves better results than an existing training approach for outpainting.

==> bmvc/content_sup/02_Experiment_settings.tex <==
% 그림 수정해야 함.
\subsection{Network Architecture}
In our main paper, except for the task with irregular masks (Section 4.4), we evaluate In-N-Out using a variant of Semantic Regeneration Network (SRN)~\cite{wang2019wide}. 
We use SRN as our base network since
%because the code was well organized, and 
it demonstrates its performance on diverse content extrapolation tasks. 
Specifically, it shows its performance 
even to extrapolation of the human body, 
texture synthesis, and morphing. 
To bring the context better from the visible region, 
SRN introduces the context normalization module and it was trained with context adversarial loss and relative spatial variant loss. 
In our work, we slightly modify SRN to accommodate not only the extrapolation task but various tasks by removing the margin mechanism 
and let the masked image go directly into the input of the network; 
it allows us to use various mask shapes as well as rectangular masks. 
The illustration of SRN~\cite{wang2019wide} is shown in Figure~\ref{fig:SRN} 
and the illustration of our variant is shown in Figure~\ref{fig:SRN_variant}.

% network structure
\begin{figure}[h]
  \includegraphics[width=\linewidth]{bmvc/figures/supplement/network/SRN.pdf}
  \caption{Semantic Regeneration Network (SRN)~\cite{wang2019wide}. This figure is brought from ~\cite{wang2019wide}.}
  \label{fig:SRN}
\end{figure}

\begin{figure}[h]
  \includegraphics[width=\linewidth]{bmvc/figures/supplement/network/variant.pdf}
  \caption{Our variant of SRN. This figure is based on ~\cite{wang2019wide}.}
  \label{fig:SRN_variant}
\end{figure}

% section:ablation_study_inpainting
% section:ablation_study_outpainting
% section:ablation_study_inpainting
%\label{subsection:beach}
%\label{subsection:irregular_mask}
%\label{subsection:env_map}

% 4.2 마스크를 잘 설명해야함
% Figure 만들기
\subsection{Masks Used in Experiments}
\begin{table}[t]
\centering
\begin{subtable}[b]{\textwidth}
\centering
\begin{tabular}{lccc}
\hline
Method                   & Easy          & Difficult           & Extreme            \\ \hline
Baseline                 & 33.83          & 52.46          & 142.40          \\
\textbf{In-N-Out} & \textbf{30.48} & \textbf{45.36} & \textbf{128.10} \\ \hline
\end{tabular}
\caption{Outpainting task results for each difficulty, on CelebA-HQ dataset~\cite{karras2017progressive}}
\label{table:region_and_fid_table}
\end{subtable}

\vspace{0.1in}

\begin{subtable}[b]{\textwidth}
\centering
\begin{tabular}{lccc}
\hline
Method & PSNR & SSIM & FID \\
\hline
SRN~\cite{wang2019wide} & 18.22 & 0.513 & - \\
Baseline (Figure~\ref{fig:SRN_variant}) & 19.46 & 0.709 & 33.30 \\
PSL~\cite{kim2021painting} & 18.78 & {\textbf{0.716}} & 35.86 \\
\textbf{In-N-Out} & {\textbf{19.52}} & 0.711 & {\textbf{30.17}} \\
\hline
\end{tabular}
\caption{Outpainting task compared to baseline(Figure~\ref{fig:SRN_variant}), on beach dataset~\cite{sabini2018painting}.}
\label{table:beach_baseline_results}
\end{subtable}
\caption{
\textbf{(a)} FID results for each difficulty on outpainting task. If the visible area is less than 20\% of a masked image, it is classified as an extreme task. Masked images with less than 40\% of the visible area are classified as difficult tasks, and others are classified as easy tasks.
\textbf{(b)} Quantitative results on outpainting task (beach dataset~\cite{sabini2018painting}). Our baseline result is added.
}
\label{table:sup_table}
\end{table}

\begin{figure}[h]
\centering
  \includegraphics[width=0.5\linewidth]{bmvc/figures/supplement/masks/distribution.pdf}
  \caption{Distribution of test mask area in Section 4.2. This represents the ratio of visible region to the image. We tested our method on masks of various sizes.}
  \label{fig:test_mask_distribution}
\end{figure}

% partial panorama images
\begin{figure}[h]
  \includegraphics[width=\linewidth]{bmvc/figures/supplement/masks/trail_images.pdf}
  \caption{Examples of partial panorama images. Up: Input of our work. Down: Input images used in lighthouse~\cite{srinivasan2020lighthouse}. We use a b-spline function with 4 random points including the center to make natural-looking partial panoramas.}
  \label{fig:trail_imgs}
\end{figure}

\begin{figure}[h]
\centering
  \includegraphics[width=0.8\linewidth]{bmvc/figures/supplement/masks/train_masks.pdf}
  \caption{Illustration of used masks.}
  \label{fig:train_masks}
\end{figure}

\Skip{
\begin{table}[t]
\centering
\begin{subtable}[b]{0.49\textwidth}
\centering
\begin{tabular}{lccc}
\hline
Method & PSNR & SSIM & FID \\
\hline
SRN~\cite{wang2019wide} & 18.22 & 0.513 & - \\
Baseline (Figure~\ref{fig:SRN_variant}) & 19.46 & 0.709 & 33.30 \\
PSL~\cite{kim2021painting} & 18.78 & {\textbf{0.716}} & 35.86 \\
\textbf{In-N-Out} & {\textbf{19.52}} & 0.711 & {\textbf{30.17}} \\
\hline
\end{tabular}
\caption{Outpainting compared to baseline(Figure~\ref{fig:SRN_variant}), on beach dataset~\cite{sabini2018painting}.}
\label{table:beach_baseline_results}
\end{subtable}
\caption{
Quantitative results on outpainting task (beach dataset~\cite{sabini2018painting}). Our baseline results are added.
}
\label{table:sup_table2}
\end{table}
}

For the outpainting task on CelebA-HQ dataset (Section 4.2), we use rectangular masks with random sizes for the test set. 
Specifically, we use face locations (used to crop) recursively to mask the cropped images,
which enables various mask sizes and ratios.
The detailed process can be found in our code.
The distribution of the test mask area are shown in Figure~\ref{fig:test_mask_distribution}, and test results according to the difficulty are shown in Table~\ref{table:region_and_fid_table}.
If the visible area is less than 20\% of a masked image, it is classified as an extreme task. Masked images with less than 40\% of the visible area are classified as difficult tasks, and others are classified as easy tasks.
%This lets us reproduce the test masks 
%easily and explore masks with various difficulty.

For environment map estimation (Section 4.5), we use a b-spline function for the masks of train set and test set; 
it makes natural-looking partial panoramas. 
The b-spline function is configured with 4 random points including the center of the image, where each point shows 60-degree FoV.
As a result, we could generate images that are similar to input images in lighthouse~\cite{srinivasan2020lighthouse}.
Note that In-N-out is trained on inverse masks, where the visible region and masked region are swapped, in training steps. 
The illustration of partial panorama images are shown in Figure~\ref{fig:trail_imgs}, and all illustrations of the train set and test set used in our experiments are shown in Figure~\ref{fig:train_masks}.

\subsection{Setup for Experiments}
% For Sec.section 4.1 and 4.2, since training iterations are not specified in the existing paper (SRN [30]), we chose (pretrain 40k0000 + train 4000040k) and (45000 45K + 4500045k) for each experiment as the loss curves are converged. For section 4.3, we chose (40000 40k+ 4000040k), and for section 4.5, we chose (45000 45k+ 4500045k). For section Sec. 4.4, we followed the training procedure specified in MEDFE [21] and Shift-Net [34] while In-N-Out does outpainting for half of the iterations. All comparisons of baselines and In-N-Out are based on the same iterations and fair experimental settings. 

For Section 4.1 and 4.2, since training iterations are not specified in the existing paper (SRN~\cite{wang2019wide}),  we chose (pretrain 40k + train 40k) and (45k + 45k) for each experiment as the loss curves are converged. For Section 4.3, we chose (40k+ 40k), and for Section 4.5, we chose (45k+ 45k). For Section 4.4, we followed the training procedure specified in MEDFE~\cite{Liu2019MEDFE} and Shift-Net~\cite{yan2018shift} (30 epochs for each baseline) while In-N-Out does outpainting for half of the iterations (15 epochs: inverse mask, 15 epochs: fine-tune).

For the experiments in Section 4.4, We follow the training and testing split of the dataset, and we use resized images to $256 \times 256$. % We train 30 epochs as \cite{Liu2019MEDFE} and \cite{yan2018shift} for baseline. For In-N-Out, we train for 15 epochs with inverse masks, then fine-tune for 15 epochs.

For the experiment in Section 4.5, we follow the official split of LAVAL Indoor HDR Dataset~\cite{10.1145/3130800.3130891}, and we use resized images to $128 \times 256$ (respectively height and width).
We use random crop, random flip, and gray-scaled images as data augmentation for our training. We use 45,000 iterations for the training steps and 45,000 iterations for the fine-tuning with batch size 4.

\subsection{Details of iterations}
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/inpainting_finetuning_InNOut_fixed2.pdf}
\caption{In, Fine-tune}
\label{in_finetuning_fid}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/inpainting_more_fid.pdf}
\caption{More from (a)}
\label{in_finetuning_more_fid}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/outpainting_finetuning_InNOut_fixed2.pdf}
\caption{Out, Fine-tune}
\label{out_finetuning_fid}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/outpainting_more_fid.pdf}
\caption{More from (c)}
\label{out_finetuning_more_fid}
\end{subfigure}

\caption{\textbf{(b)}: More iterations from Section 4.1.
\textbf{(d)}: More iterations from section 4.2.
Each graph shows FID (Fréchet inception distance)~\cite{10.5555/3295222.3295408} during each stage.}
\label{fig:full_fid2}
\vspace{-0.2in}
\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/inpainting_20000to40000_training_fid.pdf}
\caption{In, Training}
\label{in_training2_fid}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/inpainting_20000to40000_fid.pdf}
\caption{In, Fine-tune}
\label{in_finetuning_more2_fid}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/outpainting_25000to45000_fid.pdf}
\caption{Out, Fine-tune}
\label{out_finetuning2_fid}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/outpainting_25000to45000_15000more_fid.pdf}
\caption{More from (c)}
\label{out_finetuning_more2_fid}
\end{subfigure}

\caption{\textbf{(a)}-\textbf{(b)}: Section 4.1 with (N = 20000, K = 40000).
\textbf{(c)}-\textbf{(d)}: Section 4.2 with (N = 25000, K = 60000).
Each graph shows FID (Fréchet inception distance)~\cite{10.5555/3295222.3295408} during each stage.}
\label{fig:full_fid3}
\vspace{-0.2in}
\end{figure}

To choose N and K, we selected appropriate iterations to steps when the training curve is converged. For section 4.1, we found that both baseline and In-N-Out showed similar trends (as shown in Figure~\ref{fig:full_fid2}) and didn’t improve much after additional 40000 iterations. Also, for section 4.2, both baseline and In-N-Out showed similar trends after additional 50000 iterations.
Additionally, we did experiments with (Section 4.1, N=20000, K=40000), and (Section Sec. 4.2, N=25000, K=60000) as shown in Figure~\ref{fig:full_fid3}. We have consistently good results with using these different N and K.

==> bmvc/content_sup/03_More_results.tex <==
% cite 해주기
We provide test results (PSNR and SSIM) of each iteration in Figure~\ref{fig:psnr_ssim} for image inpainting and image outpainting, similar to Figure 1 in our main paper.
More visual comparisons on image inpainting, image outpainting are given in Figure~\ref{fig:inpainting_more_results}, ~\ref{fig:outpainting_more_results}, %~\ref{fig:outpainting_extreme_results}, 
and ~\ref{fig:beach_more_results}. Also, we provide our baseline for outpainting task on beach dataset in Table~\ref{table:beach_baseline_results}.

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/in_psnr_finetuning_fixed.pdf}
\caption{In, PSNR.}
\label{in_finetuning_psnr}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/in_ssim_finetuning_fixed.pdf}
\caption{In, SSIM.}
\label{in_finetuning_ssim}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/out_psnr_finetuning_fixed.pdf}
\caption{Out, PSNR.}
\label{out_finetuning_psnr}
\end{subfigure}
\begin{subfigure}[b]{0.23\linewidth}
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/out_ssim_finetuning_fixed.pdf}
\caption{Out, SSIM.}
\label{out_finetuning_ssim}
\end{subfigure}

\caption{\textbf{(a)}-\textbf{(b)}: PSNR and SSIM of each iteration in fine-tuning stage, on inpainting task.
\textbf{(c)}-\textbf{(d)}: PSNR and SSIM of each iteration in fine-tuning stage, on outpainting task. 
In-N-Out also shows better performance in terms of SSIM.}
\label{fig:psnr_ssim}
\vspace{-0.2in}
\end{figure}

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/sup_inpainting_imgs1.pdf}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/sup_inpainting_imgs2.pdf}
\end{subfigure}
\caption{More results on inpainting task (CUB200 dataset~\cite{welinder2010caltech}).}
\label{fig:inpainting_more_results}
\vspace{-0.2in}
\end{figure}

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/sup_outpainting_imgs1_fixed.pdf}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/sup_outpainting_imgs2_fixed.pdf}
\end{subfigure}
\caption{More results on outpainting task (CelebA-HQ dataset~\cite{karras2017progressive}).}
\label{fig:outpainting_more_results}
\vspace{-0.2in}
\end{figure}

\Skip{
\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/sup_extreme_imgs1.pdf}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/sup_extreme_imgs2.pdf}
\end{subfigure}
\caption{More results on outpainting task (CelebA-HQ dataset~\cite{karras2017progressive}), with extreme masks.}
\label{fig:outpainting_extreme_results}
\vspace{-0.2in}
\end{figure}
}

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.7\textwidth}
\centering
\includegraphics[width=\linewidth]{bmvc/figures/supplement/results/sup_beach_imgs.pdf}
  \caption{Outpainting task compared to PSL~\cite{kim2021painting}.}
\end{subfigure}
\caption{More results on outpainting task (beach dataset~\cite{sabini2018painting}), compared to PSL~\cite{kim2021painting}.}
\label{fig:beach_more_results}
\vspace{-0.2in}
\end{figure}

